Semifinite harmonic functions on the Gnedin-Kingman graph

We study the Gnedin-Kingman graph, which corresponds to Pieri's rule for the monomial basis $\{M_{\lambda}\}$ in the algebra $\mathrm{QSym}$ of quasisymmetric functions. The paper contains a detailed announcement of results concerning the classification of indecomposable semifinite harmonic functions on the Gnedin-Kingman graph. For these functions, we also establish a multiplicativity property, which is an analog of the Vershik-Kerov ring theorem.

==> 0_Main_results/Compositions.tex <==

\section{Введение}
В работе Кингмана \cite{kingman} были описаны  случайные перестановочно-инвариантные разбиения (random exchangeable partitions) множества натуральных чисел. Такие разбиения параметризуются вероятностными мерами на симплексе Кингмана, элементы которого суть бесконечные последовательности вещественных чисел \mbox{$(\al_1\ge \al_2\ge\dots\ge0)$} с условием \mbox{$\summ_i \al_i\le1$.} Теорему Кингмана можно переформулировать в терминах гармонических функций на некотором графе ветвления -- графе Кингмана $\king$ (\cite{versh_ker_87,kerov_vershik1990,kerov_book}). Вершины этого графа соответствуют диаграммам Юнга, а ребра отвечают правилу Пиери для мономиального базиса в алгебре симметрических функций $\sym$. 

Гнединым \cite{gnedin_97} был получен аналог теоремы Кингмана для линейно упорядоченных разбиений. Тогда, как показано в \cite{gnedin_97}, роль симплекса Кингмана играет пространство открытых подмножеств единичного интервала. Теорему Гнедина можно тоже переформулировать в терминах гармонических функций на некотором графе ветвления. Этот граф мы обозначаем через $\GK$ и предлагаем называть графом Гнедина--Кингмана. Его вершины  состоят из всевозможных композиций, а кратности ребер задаются правилом Пиери для мономиального базиса в алгебре \textit{квазисимметрических} функций $\qsym$. Эта интерпретация используется в работе Карева и Никитина \cite{karev_nikitin2018}, в которой теорема Гнедина передоказана другим методом.


Цель настоящей работы -- классифицировать неразложимые \textit{полуконечные} гармонические функции на графе Гнедина-Кингмана. Условие полуконечности предполагает, что в некоторых вершинах функция принимает значение $+\infty$; точное определение дано в параграфе $2.1$. Основной результат дается теоремой \ref{maintheorem}. Она показывает, что параметрами классификации служат конечные наборы непересекающихся интервалов в $(0,1)$ плюс некоторые дискретные данные (наборы композиций). 

Применительно к графу Кингмана задача о полуконечных гармонических функциях была решена Вершиком и Керовым \cite{kerov_example,vershik_Kerov83}. Говоря неформально, наш результат соотносится с их результатом так же, как теорема Гнедина соотносится с теоремой Кингмана. 

Используя естественное вложение колец $\sym\hookrightarrow \qsym$, можно установить некоторое соответствие  между полуконечными гармоническими функциями на графах $\GK$ и $\king$. Его точное описание дается  в предложении \ref{restriction from com to king}.

В заключение отметим, что граф $\GK$ служит диаграммой Браттели некоторой AF-алгебры, а неразложимые полуконечные гармонические функции на $\GK$ соответствуют нормальным факторпредставлениям этой алгебры типа I$_\infty$ и  II$_\infty$.




\section{Граф Гнедина-Кингмана и гармонические функции}
Граф Гнедина-Кингмана $\GK$ -- это градуированный граф $\GK=\bigsqcup\limits_{n\geq 0} \GK_n$, где $\GK_n$ --  это все возможные композиции(упорядоченные разбиения) числа $n$. По опредедению полагается $\GK_0=\{\diameter\}$.

Ребра между композициями с соседних уровней устроены следующим образом. Пусть $\mu=(n_1\lldots n_k)$, $|\mu|=N$, тогда $\mu$ соединена ребрами со всеми композициями $\nu$, $|\nu|=N-1$, которые получаются из $\mu$ 
\begin{itemize}
    \item уменьшением одного из чисел $n_i$ на единицу при $n_i\geq 2$,
    
    \item извлечением единицы из последовательности единиц, тем самым уменьшая длину этой последовательности на один: $\underbrace{(1\lldots 1)}_{j}\mapsto\underbrace{(1\lldots 1)}_{j-1}$. 
\end{itemize}

В первом случае кратность ребра равна $1$, во втором случае она равна $j$ (см. Рисунок \ref{comp graph pict}). 

\begin{remark}
Ребра в графе $\GK$ отражают правило Пьери для мономиальных квазисимметрических функций $M_{\la}$ (см. \cite[$(3.12)$]{quaisymmetric_book}  для $\al=(1)$).
\end{remark}

Если из $\nu$ в $\mu$ идет по крайней мере одно ребро, то мы пишем $\nu\nearrow \mu$. Кратность ребра, идущего из $\nu$ в $\mu$ будем обозначать через $\ka(\nu,\mu)$. По определению полагается $\ka(\nu,\mu)=0$, если $|\mu|-|\nu|\neq 1$ или же \mbox{$\nu\in\GK_{N-1}$}, \mbox{$\mu\in\GK_N$}, но $\nu$ и $\mu$ не соединены ни одним ребром.

\emph{Путем} будем называть последовательность композиций $\la_1,\la_2,\la_3,\ldots$(конечную или бесконечную) с условием $\la_i\nearrow \la_{i+1}\ \forall i$.

Будем говорить, что $\mu$ лежит выше чем $\nu$, если $\mu$ лежит на более высоком уровне чем $\nu$ и их можно соединить путем. В этом случае мы будем писать $\mu>\nu$.


\begin{figure}[h]
    \centering
    \import{0_Main_results/}{Picture_graph}
    \caption{Граф Гнедина-Кингмана}
    \label{comp graph pict}
\end{figure}

\begin{definition}
 Функция $\varphi\colon \GK\rightarrow \R_{\geq 0}\cup\{+\Inf\}$, заданная на множестве вершин графа $\GK$ называется \emph{гармонической}, если она удовлетворяет условию:
\begin{speqn}
 \varphi(\la)=\summ_{\mu:\la\nearrow \mu}\ka(\la,\mu)\varphi(\mu),\ \ \forall \la\in\GK.
\end{speqn}
\end{definition}
\begin{remark}\label{conventions}
Мы пользуемся следующими соглашениями: 
\begin{itemize}
    \item $x+\lr{+\Inf}=+\Inf,\ x\in\R$,
    
    \item $\lr{+\Inf}+\lr{+\Inf}=+\Inf$,
    
    \item $0\cdot \lr{+\Inf}=0$.
\end{itemize}  
\end{remark}

\begin{observation}
Пусть $\varphi$ -- гармоническая функция. Если $\varphi(\la)<+\Inf$, то для любой композиции $\mu$ такой, что $\mu>\la$ мы имеем $\varphi(\mu)<+\Inf$. Кроме того, если $\varphi(\la)=0$, то для любой композиции $\mu$ такой, что $\mu>\la$ мы имеем $\varphi(\mu)=0$.
\end{observation}

\begin{definition}
Множество всех \mbox{$\la\in\GK$}, для которых \mbox{$\varphi(\la)<+\Inf$} мы будем называть \emph{идеалом конечности} $\varphi$. \emph{Идеал нулей} $\varphi$ будет обозначаться через $\ker{\varphi}$, а \emph{носитель} $\{\la\in\GK\mid \varphi(\la)>0\}$ через $\supp{\varphi}$.
\end{definition}
\begin{remark}
Такие названия обусловлены тем, что множество вершин $I\subset \GK$, удовлетворяющих свойству \mbox{$\la\in I,\ \mu>\la\implies \mu\in I$}, принято называть \textit{идеалом} в графе ветвления \cite{kerov_vershik1990}.
\end{remark}

\begin{definition}
 Гармоническая функция $\varphi$ называется \emph{конечной}, если \mbox{$\varphi(\la)<+\Inf, \forall \la\in\GK$.}
\end{definition}

\begin{remark}
Конечные гармонические функции предполагаются нормированными: \mbox{$\varphi(\diameter)=1$.}
\end{remark}

\begin{definition}
 Конечная гармоническая функция $\varphi$ называется \emph{неразложимой}, если для любых конечных гармонических функций $\varphi_1,\varphi_2$ и положительных вещественных чисел $c_1,c_2$ таких, что \mbox{$c_1+c_2=1$} мы имеем \mbox{$\varphi=c_1\varphi_1+c_2\varphi_2\ \implies \varphi=\varphi_1\ \text{или}\ \varphi=\varphi_2$}.
\end{definition}

По каждой конечной гармонической функции $\varphi$ можно построить функционал $F_{\varphi}\colon\qsym\rightarrow \R$:
\begin{speqn}
 F_{\varphi}\lr{M_{\la}}=\varphi(\la),
\end{speqn}
где $M_{\la}$ мономиальная квазисимметрическая функция \cite{quaisymmetric_book}.

Такой функционал удовлетворяет следующим свойствам:
\begin{enumerate}
    \item\label{11} $F_{\varphi}\lr{M_{\la}}\geq 0$,
    
    \item\label{22} $F_{\varphi}\lr{M_{(1)}M_{\la}}=F_{\varphi}\lr{M_{\la}}$,
    
    \item\label{33} $F_{\varphi}\lr{1}=1$.
\end{enumerate}

\begin{proposition}
Cоответствие $\varphi\longleftrightarrow F_{\varphi}$ задает биекцию между конечными гармоническими функциями $\GK$ и функционалами $\qsym\rightarrow \R$, удовлетворяющими свойствам \eqref{11},\eqref{22},\eqref{33}.
\end{proposition}

Мы будем отождествлять $\varphi$ и $F_{\varphi}$ и использовать для них одинаковое обозначение -- $\varphi$.


\begin{theorem}[Теорема о кольце Вершика-Керова]\cite[Proposition 8.4]{gnedin_olsh2006}
Конечная гармоническая функция $\varphi$ на графе $\GK$ неразложима тогда и только тогда, когда она задает мультипликативный функционал: $\varphi\lr{a\cdot b}=\varphi\lr{a}\cdot \varphi\lr{b}\ \forall a,b\in\qsym$.
\end{theorem}

\subsection{Полуконечные гармонические функции и аддитивные \mbox{$\R_{\geq 0}$} -- линейные отображения \mbox{$K\rightarrow \R_{\geq0}\cup\{+\Inf\}$}}
\phantom{}

Рассмотрим алгебру \mbox{$R=\quotid{\qsym}{M_{(1)}-1}$} и положительный конус \mbox{$K\subset R$}, натянутый на образы мономиальных квазисимметрических функций: \mbox{$K=\span{\R_{\geq0}}{\left[M_{\la}\right]\mid \la\in\GK}$}, где $[\ \cdot\ ]\colon\qsym\twoheadrightarrow R$ -- канонический гомоморфизм. Отметим, что этот конус замкнут относительно умножения: $K\cdot K\subset K$. Конус $K$ задает частичный порядок $\geq_K$ на алгебре $R$: $a\geq_K b\iff a-b\in K$.

Каждая гармоническая функция $\varphi$ задает аддитивное $\R_{\geq0}$ -- линейное отображение $F_{\varphi}\colon K\rightarrow \R_{\geq0}\cup\{+\Inf\}$:
\begin{speqn}
 F_{\varphi}\lr{\left[M_{\la}\right]}=\varphi(\la).
\end{speqn}

Напомним, что мы пользуемся соглашением $0\cdot\lr{+\Inf}=0$, см. Замечание \ref{conventions}.

\begin{definition}
Гармоническая функция $\varphi$ называется \emph{полуконечной}, если она не является конечной и отображение \mbox{$F_{\varphi}\colon K\rightarrow \RR\cup\{+\Inf\}$} обладает следующим свойством полунепрерывности снизу
\begin{speqn}\label{lower semicont}
F_{\varphi}(a)=\sup_{\substack{b\in K\colon  b\leq_K a,\\ F_{\varphi}(b)<+\Inf}}F_{\varphi}(b),\ \ \ \ \ \forall a\in K. 
\end{speqn}
\end{definition}
\begin{observation}
Если \mbox{$F_{\varphi}(a)<+\Inf$}, то условие \eqref{lower semicont} превращается в тривиальное равенство \mbox{$F_{\varphi}(a)=F_{\varphi}(a)$.}
\end{observation}
\begin{remark}\label{remark 321}
 Гармоническая функция $\varphi$ является полуконечной тогда и только тогда, когда существует \mbox{$a\in K$} такое, что \mbox{$F_{\varphi}(a)=+\Inf$} и для любого такого $a$ найдется последовательность \mbox{$\{a_n\}_{n\geq 1}\subset K$} такая, что \mbox{$a_n\leq_K a$}, \mbox{$F_{\varphi}(a_n)<+\Inf$} и  \mbox{$\lim\limits_{n\to+\Inf}F_{\varphi}(a_n)=+\Inf$.} 
\end{remark}
\begin{remark}
Если $\varphi$ полуконечная гармоническая функция $\GK$, то найдется \mbox{$\la\in\GK$} такая, что $\varphi(\la)=+\Inf$ и для любой такой $\la$ найдется вершина $\mu> \la$ такая, что \mbox{$0<\varphi(\mu)<+\Inf$.}
\end{remark}

\begin{proposition}
Cоответствие $\varphi\longleftrightarrow F_{\varphi}$ задает биекцию между полуконечными гармоническими функциями на графе $\GK$ и $\R_{\geq0}$ -- линейными аддитивными отображениями $K\rightarrow \RR\cup\{+\Inf\}$, удовлетворяющими свойству \eqref{lower semicont}.
\end{proposition}

Мы будем отождествлять $\varphi$ и $F_{\varphi}$ и использовать для них одинаковое обозначение -- $\varphi$.

\begin{definition}
 Полуконечная гармоническая функция $\varphi$ называется \emph{неразложимой}, если для любой конечной (тождественно не равной нулю) или полуконечной гармонической функции $\varphi'$ такой, что $\varphi\geq \varphi'$,  мы имеем $\varphi=c\varphi'$ для некоторого $c\in\R$.
\end{definition}

\begin{theorem}\cite[p.144]{vershik_Kerov83}\label{property mult}
Пусть $\varphi$ -- полуконечная неразложимая гармоническая функция $\zig$. Тогда существует $\psi$, конечная неразложимая гармоническая функция на $\zig$, такая, что для любого \mbox{$a\in K$} и любого \mbox{$b\in K$} такого, что \mbox{$\varphi(b)<+\Inf$} выполнено равенство \mbox{$\varphi(a\cdot b)=\psi(a)\cdot \varphi(b)$.}
\end{theorem}

\begin{comment}
\begin{remark}
Равенство \eqref{property mult eq} мы будем называть свойством мультипликативности полуконечных гармонических функций. Заметим, однако, что из свойства мультипликативности не следует, что соответсвующая полуконечная гармоническая функция является неразложимой. 
\end{remark}
\end{comment}


\section{Конечные гармонические функции на графе Гнедина-Кингмана}
Опишем неразложимые конечные гармонические функции на графе Гнедина-Кингмана с непустым множеством нулей \cite{karev_nikitin2018}.

\begin{definition}
 Пусть $U_0$ множество всевозможных открытых подмножеств единичного интервала, состоящих из конечного объединения интервалов, общая длина которых равна единице. Интервалы разделяются на два типа: \textit{$h$ - интервалы} и \textit{$v$ - интервалы}($h$ от horizontal, а $v$ от vertical). Два $v$ - интервала не могут идти подряд, а $h$ - интервалы могут.
\end{definition}

\begin{remark}
Аналогом $v$ - интервалов в графе Кингмана является параметр \mbox{$\ga=1-\summ_{i}\al_i$}, поэтому они будут обоначаться символом $\ga$ с индексом, а $h$ - интервалы -- символом $u$ с индексом.
\end{remark}


\begin{remark}
Графически $h$ - интервалы будут изображаться синими отрезками, окруженными круглыми скобками, $v$ - интервалы будут изображаться черными отрезками без каких-либо скобок.
\end{remark}

\begin{example}\label{example2}
Следующий элемент \mbox{$u\in U_0$} состоит из четырех $h$ - интервалов -- $u_1,u_2,u_3,u_4$ и двух $v$ - интервалов -- $\ga_1,\ga_2$:
\begin{figure}[H]
    \centering
    \import{0_Main_results/}{Picture1_1}
\end{figure}
\end{example}

 Каждому элементу \mbox{$u\in U_0$} соответствует конечная гармоническая функция $\varphi_u$ на графе Гнедина-Кингмана $\GK$ \cite{gnedin_97}. Описание $\varphi_u$ будет очень похоже на конструкцию Керова границы графа Юнга: \cite[p. 13-18]{gnedin_olsh2006} и особенно \cite[p.18-19 Remark 4.8]{gnedin_olsh2006}.
 
 Для того, чтобы явно задать $\varphi_u$ нам понадобятся следующие два гомоморфизма $\psi_+,\psi_-\colon \qsym\rightarrow \R$, заданных по правилам:
    \begin{speqn}\label{psi}
    \psi_+(M_{\la})=\begin{cases}
    1,\ \text{если}\ \la=(n),\\
    
    0,\ \text{иначе},
    \end{cases}\ \ \ \psi_-(M_{\la})=\begin{cases}
    \cfrac{1}{n!}\ ,\ \text{если}\ \la=(\underbrace{1,\ldots,1}_n),\\
    
    0,\ \text{иначе}.
    \end{cases}
    \end{speqn}
    
Пусть $u$ состоит в сумме из $m$ интервалов. Каждому из $h$ - интервалов поставим в соответствие $\psi_+$, а каждому из $v$ - интервалов -- $\psi_-$. Тогда мы получим набор гомоморфизмов $\psi_1,\ldots, \psi_m\colon \qsym\rightarrow \R$.  
    
Для вещественного числа $t\neq 0$ обозначим через $r_t$ автоморфизм $\qsym$, заданный по правилу $M_{\la}\mapsto t^{|\la|}M_{\la}$. 
    
Через $\Delta$ обозначается коумножение в алгебре $\qsym$,
\begin{comment}:
\begin{speqn}
    \Delta \left(M_{\la}\right)=\summ_{\la=\mu\sqcup\nu}M_{\mu}\otimes M_{\nu},
\end{speqn}
\end{comment}
а $\Delta^{(n)}\colon \qsym\rightarrow \qsym^{\otimes n}$ определяется индуктивно: 
\begin{speqn}
 \Delta^{(n+1)}=\lr{\Delta\otimes 1}\circ \Delta^{(n)}=\lr{1\otimes\Delta}\circ \Delta^{(n)},\ \  \Delta^{(2)}=\Delta.
\end{speqn}

\begin{comment}
Тогда 
\begin{speqn}
 \Delta^{(n)} \left(M_{\la}\right)=\summ_{\substack{\la_1,\ldots,\la_n\in \GK:\\ \la=\la_1\sqcup\ldots \sqcup\la_n}} M_{\la_1}\otimes M_{\la_2}\otimes \ldots \otimes M_{\la_n}.
\end{speqn}
\end{comment}
Обозначим через $w=(w_1,\ldots, w_m)$ набор длин интервалов $u$, взятых в естественном порядке слева направо. 

Гармоническая функция $\varphi_u$ определяется следующим образом:
\begin{speqn}\label{formula1}
 \varphi_u(\la)=\lr{\psi_1\otimes\ldots\otimes \psi_m}\circ \lr{r_{w_1}\otimes \ldots \otimes r_{w_m}}\circ \Delta^{(m)}\lr{M_{\la}}.
\end{speqn}

\begin{comment}
Можно написать и более явную формулу:
\begin{speqn}\label{formula2}
 \varphi_u(\la)=\summ_{\substack{\la_1,\ldots,\la_m\in \GK:\\ \la=\la_1\sqcup\ldots \sqcup\la_m}} w_1^{|\la_1|}\ldots w_m^{|\la_m|}\ \cdot \psi_1\lr{M_{\la_1}} \psi_2\lr{M_{\la_2}}\ldots \psi_m\lr{M_{\la_m}}.
\end{speqn}

\begin{remark}
Ненулевой вклад в правой части \eqref{formula2} дадут лишь те слагаемые, которые удовлетворяют следующему требованию: если $i$ - ый элемент в $u$ является интервалом, то $\la_i$ -- строка произвольной длины, если же $i$ - ый элемент в $u$ является отрезком, то $\la_i$ -- столбец.
\end{remark}
\end{comment}
\begin{remark}\label{important rem}
При каждом фиксированном $\la$ правая часть \eqref{formula1} задает некоторую функцию на $U_0$, которую мы будем обозначать через $\M_{\la}(u)$.
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{speqn}\label{formula1}
    M^{\circ}_{\la}(u)=\overset{\longrightarrow}{\bigotimes\limits_{s\in el(u)}}\psi_{\eps(s)}\circ \overset{\longrightarrow}{\bigotimes\limits_{s\in el(u)}} r_{|s|}\circ  \Delta^{(2k+1)}\lr{M_{\la}}
\end{speqn}


\lr{\psi_{-}\otimes \psi_{+}\otimes \psi_{-}\otimes\ldots\otimes \psi_{+}\otimes \psi_{-}}\circ
    \lr{r_{\ga_0}\otimes r_{u_1}\otimes r_{\ga_1}\otimes\ldots\otimes r_{u_k}\otimes  r_{\ga_k}}\circ


или

\begin{speqn}\label{formula2}
     M^{\circ}_{\la}(u)=\summ_{\substack{p_0,\ldots, p_k\geq 0,\\ q_1,\ldots, q_k\geq 0, \\ (1^{p_0},q_1,1^{p_1},q_2,\ldots,q_k,1^{p_k})=\la}}\cfrac{\ga_0^{p_0}}{p_0!}\cdot \cfrac{\ga_{1}^{p_1}}{p_1!}\cdot\ldots\cdot \cfrac{\ga_{k}^{p_k}}{p_k!}\cdot u_1^{q_1}u_2^{q_2}\ldots u_k^{q_k} .
\end{speqn}  

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Опишем множество вершин $\supp{\varphi_u}$, на которых $\varphi_u$ принимает ненулевое значение. Для этого нам понадобится некоторая "бесконечная" композиция.
\begin{definition}
 \emph{Бесконечной композицией} $\GK_u$, соответствующей \mbox{$u\in U_0$}, мы будем называть последовательность из строк и столбцов бесконечной длины. Строки соответствуют $h$ - интервалам $u$, а столбцы -- $v$ - интервалам. Строки и столбцы в бесконечной композиции идут в том же порядке, в котором шли $h$ - интервалы и $v$ - интервалы в $u$. Мы будем отождествлять эту бесконечную композицию с множеством (обычных) композиций, содержащихся внутри нее, и обозначать это множество тем же символом $\GK_u$. Таким образом, каждая композиция из $\GK_u$ может быть представлена в виде последовательного объединения строк и столбцов произвольной(быть может, нулевой) длины с тем условием, что строки соответствуют $h$ - интервалам $u$, а столбцы $v$ - интервалам.
\end{definition}

\begin{figure}[h]
    \centering
    \import{0_Main_results/}{Picture1}
    \caption{$\GK_u$ для \mbox{$u\in U_0$} из примера \ref{example2}.}
    Строки и столбцы из белых клеток имеют бесконечную длину.
    \label{pict2}
\end{figure}

\begin{remark}
Бесконечная композиция $\GK_u$ никак не зависит от длин интервалов, но зависит от их взаимного расположения. 
\end{remark}


\begin{proposition}
$\supp{\varphi_u}=\GK_u$.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
C каждой конечной гармонической функцией $\varphi$ на графе $\GK$ можно связать вероятностную меру $P_{\varphi}$ на пространстве путей. Пусть $\T$ -- множество бесконечных путей, а $\T_n$ -- конечные пути, заканчивающиеся на  $n$ - ом уровене. Пусть также $\pi_n\colon \T\rightarrow \T_n$ -- естесственная проекция, забывающая все вершины в бесконечном пути, находящиеся на уровне $n+1$ и выше. Мера $P_{\varphi}$ задается на цилиндрических множествах -- $\pi^{-1}_n\lr{X}$, где $X\subset\T_n$. Пусть $t_n\in\T_n$ заканчивается в $\la\in\GK$, тогда по определению полагается $P_{\varphi}\lr{\pi^{-1}_n\lr{t_n}}=\varphi\lr{\la}$. В частности, вероятность того, что случайный путь проходит через вершину $\la$ равна $\dim_{\GK}(\la)\cdot\varphi(\la)$. Обозначим через $P_u$ меру на пространстве путей, соответсвующую $\varphi_u$. Имея эту меру, мы можем рассматривать случайные пути в графе $\GK$. Тогда типичный путь(не лежащий ни в каком измеримом множестве меры нуль) в смысле $P_u$ будет лежать внутри $\GK_u$. Такой путь будет заполнять всю бесконечную композицию $\GK_u$ в том смысле, что начиная с некоторого момента, композиции из нашего пути будут состоять из стольких же строк и стольких же столбцов, сколько их есть в $\GK_u$ и, кроме того, эти строки и столбцы будут неограниченно расти. Внутри композиций из нашего пути эти строки и столбцы будут расположены в таком же порядке как и в $\GK_u$.  Можно считать, что $\GK_u$ -- это, как бы, профиль такого пути. Кроме того, частоты появления новых клеток в строках и столбцах композиций из типичного пути задаются наборами чисел $u$ и $\ga$ соответственно. Тут под $u$ понимается только лишь набор длин интервалов элемента $U_0$, а не сам этот элемент. Неудачное обознаение, но злоупотреблять мы им не будем. 
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \section{Основные результаты}
 Теперь мы опишем неразложимые полуконечные гармонические функции $\varphi_{\wt{u}}$, соответствующие $\wt{u}\in \wt{U}_0$. Мы приведем два эквивалентных описания $\varphi_{\wt{u}}$.
 
\begin{definition}
 Рассмотрим множество $\wt{U}_0$, состоящее из всевозможных наборов $(u,\ga;\la_0,\la_1\ldots,\la_m)$, где 
 \begin{itemize}
     \item \mbox{$u, \ga$} -- открытые непересекающиеся подмножества единичного интервала, состоящие из несвязного объединения конечного числа интервалов, общая длина которых равна единице. Интервалы из $u$ называются \textit{$h$ - интервалами}, а интервалы из $\ga$ называются \textit{$v$ - интервалами}. 
     
     \item $m$ -- общее число интервалов $u$ и $\ga$;
     
     \item $\la_i$ -- некоторые композиции; хотя бы одна из них непустая. Мы считаем, что эти композиции находятся в граничных точках $h$ - интервалов и $v$ - интервалов. Таким образом, $\la_0$ находится в начале единичного отрезка, а $\la_m$ -- в конце. Если два $v$ - интервала идут подряд, то композиция, разделяющая их, обязательно непустая. Кроме того, композиция, стоящая рядом с $v$ - интервалом не может касаться его числом $1$, то есть, крайний со стороны $v$ - интервала символ в композиции должен быть не меньше двух. Композиции $\la_i$ будут называться \textit{разделяющими композициями}.
 \end{itemize} 
\end{definition} 

\begin{example}\label{example1}
  Следующий элемент $\wt{u}\in\wt{U}_0$ состоит из четырех $h$ - интервалов -- $u_1, u_2, u_3,u_4$ и трех $v$ - интервалов -- $\ga_1,\ga_2,\ga_3$. Последние два $v$ - интервала находятся рядом друг с другом, но разделены композицией $(3,1,5)$. 
\begin{figure}[H]
    \centering
    \import{0_Main_results/}{Picture2_1}
\end{figure}
В этом случае $m=7$ и композиции $\la_i$ следующие:
  \begin{speqn}
   \la_0=(1,1,1),\ \la_1=\diameter,\ \la_2=(5,3),\ \la_3=(1,3),\ \la_4=\la_5=\diameter,\ \la_6=(3,1,5),\ \la_7=\diameter.
  \end{speqn}
\end{example}



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{comment}
 Следует отметить, что,  в отличие от графа Кингмана, идеал конечности не всегда порождается одной композицией.  
 \newpage
 Действительно, возьмем следующий элемент $\wt{u}\in\wt{U}_0$, состоящий из одного лишь промежутка:
 \begin{figure}[h]
     \centering
     \import{0_Main_results/}{Picture_example}
 \end{figure}
 
 Легко проверить, что $\GK^{\wt{u}}$ порождается композициями -- $(1,2)$ и $(4)$, тогда мы получим, что идеал конечности $\varphi_{\wt{u}}$ порождается композициями $(1,2)$ и $(3)$. Очевидно, что он не может порождаться какой-либо одной композицией.
 \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Рассмотрим один частный случай. Пусть $\wt{u}\in \wt{U}_0$ не содержит двух подряд идущих промежутков, разделенных некоторой композицией. Если мы отбросим все разделяющие композиции, то никакие два промежутка не окажутся рядом. Обозначим результат удаления всех разделяющих композиций из $\wt{u}$ через $\ol{u}\in U_0$. Тогда у нас имеется биекция между вершинами следующих графов $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}\simeq \Pas_m\simeq \lr{\GK_{\ol{u}}}^{\la_{\ol{u}}}$. Обозначим сквозное отображение слева направо через $\la\mapsto \la^{min}$. Оно заключается в том, что мы отбрасываем все конечные наросты, которые соответствуют разделяющим композициям $\wt{u}$, а также мы добавлем по одной клетке к тем строкам, которые оказались рядом со столбцом, но раньше они с ним не соседствовали. На рисунке \ref{fig2}, такая строка также есть, хотя этот элемент $\wt{u}$ содержит два столбца разделенных композицией. Строка, о которой идет речь, находится между вторым и третьим блоком из серых клеток. После удаления этих серых блоков, строка окажется рядом со столбцом, но раньше они были разделены композицией $(5,3)$. 

В этом случае гармоническую функцию $\varphi_{\wt{u}}$ можно задать равенством

\begin{speqn}\label{def2}
 \varphi_{\wt{u}}(\la)=\begin{cases}
 M^{\circ}_{\la^{min}}(\ol{u}), &\text{если}\ \la\in \GK^{\la_{\wt{u}}}\cup \GK^{\wt{u}},\\
 +\Inf, &\text{иначе}.
 \end{cases}
\end{speqn}

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Первое описание $\varphi_{\wt{u}}$ и основная теорема}
Для того, чтобы явно описать $\varphi_{\wt{u}}$ мы отдельно опишем множество $\supp{\varphi_{\wt{u}}}$ и идеал конечности $\varphi_{\wt{u}}$. После этого мы зададим $\varphi_{\wt{u}}$ на тех композициях, которые одновременно лежат в $\supp{\varphi_{\wt{u}}}$ и идеале конечности $\varphi_{\wt{u}}$.

Мы опишем $\supp{\varphi_{\wt{u}}}$ по аналогии с конечными гармоническими функциями. Для них мы по каждому $u\in U_0$ построили бесконечную композицию $\GK_{u}$ и множество $\supp{\varphi_u}$ состояло из всех композиций, содержащихся внутри $\GK_u$. 

\begin{definition}
 \emph{Бесконечной композицией} $\GK_{\wt{u}}$, соответствующей \mbox{$\wt{u}\in \wt{U}_0$}, мы будем называть последовательность из строк и столбцов бесконечной длины, а также обычных композиций. Строки соответствуют $h$ - интервалам, бесконечные столбцы -- $v$ - интервалам, а конечные композиции -- разделяющим композициям $\wt{u}$. Бесконечные строки, бесконечные столбцы и конечные композиции идут в $\GK_{\wt{u}}$ в том же порядке, в котором шли $h$ - интервалы, $v$ - интервалы и разделяющие композиции в $\wt{u}$. Мы будем отождествлять эту бесконечную композицию с множеством композиций, содержащихся внутри нее, и обозначать это множество тем же символом $\GK_{\wt{u}}$. 
\end{definition}

По определению полагается $\supp{\varphi_{\wt{u}}}=\GK_{\wt{u}}$.
 
Для того, чтобы описать идеал конечности $\varphi_{\wt{u}}$ нам понадобится специальная композиция $\la_{\wt{u}}$. Будем говорить, что $h$ - интервал \textit{соседствует} с $v$ - интервалом, если они находятся рядом и разделены пустой композицией. Композиция $\la_{\wt{u}}$ строится следующим образом: мы берем $\wt{u}$ и на месте каждого $h$ - интервала пишем $1$, если он не соседствовал с $v$ - интервалом и $2$ в противном случае, разделяющие композиции не изменяются. После этого мы считываем все числа, которые у нас получились(числа соответствующие $h$ - интервалам и разделяющим композициям) слева направо и обозначаем результат через $\la_{\wt{u}}$. 


По определению полагается, что идеал конечности $\varphi_{\wt{u}}$ состоит из всех композиций, которые находятся выше чем $\la_{\wt{u}}$ (то есть $\geq\la_{\wt{u}}$) или не лежат в $\GK_{\wt{u}}$.

\begin{figure}[h]
      \centering
      \import{0_Main_results/}{Picture2}
      \caption{$\GK_{\wt{u}}$ для $\wt{u}$ из примера \ref{example1}}
      Белые клетки обозначают бесконечные строки и столбцы, а серые -- композиции конечного размера. Композиция $\la_{\wt{u}}$ обозначена заштрихованными клетками.
      \label{fig2}
 \end{figure}

 Мы описали идеал конечности и множество нулей $\varphi_{\wt{u}}$. Дальнейшего внимания достойно лишь множество всех композиций, которые одновременно лежат внутри $\GK_{\wt{u}}$ и содержат $\la_{\wt{u}}$. Обозначим это множество через \mbox{$\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}$}.
 
 Композиции из $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}$ естественным образом отождествляются с вершинами пирамиды Паскаля $\Pas_{m}$, где $m$ -- число интервалов в $\wt{u}$. Дело в том, что композиция $\la_{\wt{u}}$ может расти внутри $\GK_{\wt{u}}$ очень ограниченным образом -- расти могут только строки и столбцы, соответствующие $h$ - интервалам и $v$ - интервалам из $\wt{u}$. Обозначим отображение вершин $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}\iso \Pas_m$ через $\la\mapsto\la_{\pm}$. Это отображение заключается в том, что композиции, лежащей выше $\la_{\wt{u}}$, мы сопоставляем набор длин "наростов" на строках и столбцах $\la_{\wt{u}}$, соответствующих $h$ - интервалам и $v$ - интервалам. Эти длины "наростов" записываются в $\la_{\pm}$ в естесственном порядке -- слева направо, если говорить об интервалах, или сверху вниз, если говорить о бесконечной композиции $\GK_{\wt{u}}$. Набор чисел $\la_{\pm}$ мы можем разбить на два поднабора –- числа соответствующие $h$ - интервалам и $v$ - интервалам. Первый набор чисел обозначим через $\la_+$, а второй через $\la_-$. 
 
 \begin{figure}[h]
     \centering
     \import{0_Main_results/}{Picture_4}
     \caption{"Наросты" на композиции $\la_{\wt{u}}$ внутри $\GK_{\wt{u}}$ для $\wt{u}$ из примера \ref{example1}.}
     Композиция $\la_{\wt{u}}$ обозначена заштрихованными клетками. Композиция $\la$ состоит из заштрихованных, синих и оранжевых клеток. Наборы чисел $\la_+=(3,9,0,4)$, $\la_-=(4,0,2)$ и $\la_{\pm}=(3,4,9,0,4,0,2)$ -- это наборы из длин синих, оранжевых, а также и тех и других строк соответственно. Притом, если внутри белой строки или белого столбца не окажется закрашенных клеток, то на соответствующем месте в $\la_{\pm}$, а также $\la_+$ или $\la_-$ пишется ноль. 
     \label{figg3}
 \end{figure}
  
 Для элемента $\wt{u}\in\wt{U}_0$ символами $u$ и $\ga$ обозначаются наборы длин $h$ - интервалов и $v$ - интервалов.
 \begin{definition}
  \begin{speqn}\label{def111}
 \varphi_{\wt{u}}(\la)=\begin{cases}
 \cfrac{\ga^{\la_-}}{\la_-!}\ u^{\la_+}, &\text{если}\ \la\in \lr{\GK_{\wt{u}}}^{\la_{\wt{u}}},\\
 +\Inf, &\text{если}\ \la\in \GK_{\wt{u}}\backslash\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}},\\
  0, &\text{если}\ \la\notin \GK_{\wt{u}}.
 \end{cases}
\end{speqn}
Мы пользуемся обозначениями $x^{\mu}=x_1^{\mu_1}x_2^{\mu_2}\ldots$ и $x!=x_1!x_2!\ldots$ для $x=\lr{x_1,x_2,\ldots}$.

 \end{definition}
 
\begin{proposition}
Функция $\varphi_{\wt{u}}$ является неразложимой, полуконечной и гармонической. 
\end{proposition}

\begin{theorem}\label{maintheorem}
     Если $\varphi$ -- полуконечная неразложимая гармоническая функция на графе Гнедина-Кингмана $\GK$, то $\varphi$ пропорциональна  $\varphi_{\wt{u}}$ для некоторого $\wt{u}\in \wt{U}_0$.
 \end{theorem}

 \subsection{Второе описание $\varphi_{\wt{u}}$}
 Пусть $\wt{u}\in \wt{U}_0$ и $\eps$ вещественное положительное число. Обозначим через $u^{\eps}$ открытое подмножество вещественной прямой, которое получается из $\wt{u}$ следующим образом: вместо каждой разделяющей композиции мы внедряем столько интервалов длины $\eps$, какова была длина композиции. Длины $h$ - интервалов и $v$ - интервалов при этом не меняются, но сами интервалы немного сдвигаются(не имеет значения в какую сторону от точки, в которую мы внедрили $\eps$ - интервал).
 
 \begin{example}\label{example22}
  $u^{\eps}$ для $\wt{u}\in\wt{U}_{0}$ из примера \ref{example1}:
\begin{figure}[H]
    \centering
    \import{0_Main_results/}{Picture_2_epsilon}
\end{figure}
\end{example}
\begin{remark}
Переход от $\wt{u}$ к $u^{\eps}$ соответствует тому, что мы на Рис.\ref{fig2} заменяем все серые заштрихованные строки на бесконечные строки из белых клеток и, тем самым, получаем $\GK_{u^{\eps}}$.
\end{remark}
 \begin{remark}
Отметим, что $u^{\eps}$ уже не будет подмножеством единичного интервала, однако, правая часть в формуле \eqref{formula1}, по-прежнему, имеет смысл. Таким образом, определено выражение $\M_{\la}(u^{\eps})$. Кроме того, $\{\la\in\GK\mid M^{\circ}_{\la}(u^{\eps})>0\}=\GK_{u^{\eps}}$.
\end{remark}

Пусть $\wt{u}=(u,\ga;\la_0,\la_1\ldots,\la_m)$. Введем обозначение $n(\wt{u})=|\la_0|+|\la_1|+\ldots+|\la_m|$. 
\begin{proposition}\label{prop11}
\begin{speqn}\label{eq11}
 \varphi_{\wt{u}}(\la)=\begin{cases}
 \lim\limits_{\varepsilon\to 0}\cfrac{1}{\eps^{n(\wt{u})}}\cdot M^{\circ}_{\la}(u^{\eps}), &\text{если}\ \la\supseteq\la_{\wt{u}},\\
 0, &\text{если}\ \la\notin\GK_{\wt{u}},\\
 +\Inf, &\text{иначе.}
 \end{cases}
 \end{speqn}
\end{proposition}
\begin{remark}
В правой части формулы \eqref{eq11} первый и второй случай могут пересекаются. В предложении \ref{prop11} утверждается, в частности, что \mbox{$\lim\limits_{\varepsilon\to 0}\cfrac{1}{\eps^{n(\wt{u})}}\cdot M^{\circ}_{\la}(u^{\eps})=0$,} \mbox{если $\la\notin\GK_{\wt{u}}$ и $\la\supseteq \la_{\wt{u}}$.}
\end{remark}

\begin{example}
 Давайте посчитаем предел из формулы \eqref{eq11} для следующего $\wt{u}\in\wt{U}_0$.
 \begin{figure}[H]
     \centering
     \import{0_Main_results/}{Picture_5}
 \end{figure}
 
 В этом случае $u^{\eps}$ имеет вид 
 \begin{figure}[H]
     \centering
     \import{0_Main_results/}{Picture_7}
 \end{figure}
 
 Кроме того, $\la_{\wt{u}}=(3,1,1)$ и $\GK_{\wt{u}}$, $\GK_{u^{\eps}}$ имеют следующий вид. Заштрихованными клетками обозначена композиция $\la_{\wt{u}}$.
 \begin{figure}[H]
     \centering
     \import{0_Main_results/}{Picture_6}
 \end{figure}
 
 Далее мы предполагаем, что $\la\supseteq (3,1,1)$. 
 \begin{itemize}
     \item Если $\la\notin \GK_{u^{\eps}}$, то $\M_{\la}(u^{\eps})=0$.
     
     \item  Если $\la\in \GK_{u^{\eps}}$, то $\la=(n,m,k)$ при $n\geq 3,m,k\geq 1$. Тогда из формулы \eqref{formula1} имеем $\M_{\la}(u^{\eps})=\eps^{n+m}$ и
 \begin{speqn}
  \lim\limits_{\varepsilon\to 0}\cfrac{1}{\eps^{n(\wt{u})}}\cdot M^{\circ}_{\la}(u^{\eps})=\lim\limits_{\varepsilon\to 0}\eps^{n-3+m-1}=\begin{cases}
  1,\ &\text{если}\ n=3, m=1\\
  0,\ &\text{иначе}.
  \end{cases}
 \end{speqn}
 \end{itemize}

 Таким образом,
 \begin{speqn}
  \lim\limits_{\varepsilon\to 0}\cfrac{1}{\eps^{n(\wt{u})}}\cdot M^{\circ}_{\la}(u^{\eps})=\begin{cases}
  1,\ &\text{если}\ \la=(3,1,k),\ k\geq 1,\\
  0,\ &\text{если}\ \la\notin\GK_{\wt{u}},\ \la\supseteq(3,1,1).
  \end{cases}
 \end{speqn}
 
\end{example}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{comment}
 Полуконечная гармоническая функция $\varphi_{\wt{u}}$ задает вероятностную меру на пространстве путей в графе $\GK^{\la_{\wt{u}}}$, всех композиций, содержащих $\la_{\wt{u}}$. И мы можем говорить о типичных путях в смысле этой меры. Очевидно, что типичный путь обязан целиком лежать внутри $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}$. Таким образом, профиль пути начинает вырисовываться не с какого-то достаточно большого уровня(как в случае с конечными характерами) в графе $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}$, а в самом начале пути. Благодаря изоморфизму диаграмм Браттели $\lr{\GK_{\wt{u}}}^{\la_{\wt{u}}}\simeq \Pas_m$, о котором говорилось выше, мы однозначно определяем строки и столбцы композиций, которые могут расти, все же остальные будут заморожены. На рисунке \ref{fig2} замороженные строки выделены серым цветом, а растущие белым. Белые строки и столбцы неограниченно растут и, кроме того, наборы чисел $u$ и $\ga$ задают интенсивности появления новых клеток в соответствующих строках и столбцах.
 \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Мультипликативность функций $\varphi_{\wt{u}}$}
 Теперь опишем конечную гармоническую функцию на графе $\GK$, возникающую в свойстве мультипликативности для полуконечных неразложимых гармонических функций (Теорема \ref{property mult}). Обозначим через $\ol{u}$ открытое подмножество единичного интервала, которое получается из \mbox{$\wt{u}\in \wt{U}_0$} грубым отбрасыванием всех разделяющих композиций. При таком отбрасывании $v$ - интервалы, стоящие рядом склеиваются в один, а $h$ - интервалы -- нет. 
 
 \begin{example}
   Множество $\ol{u}$ для $\wt{u}\in\wt{U}_0$ из примера \ref{example1} совпадает с $u\in U_0$ из примера \ref{example2} для подходящих длин $h$ - интервалов и $v$ - интервалов. В частности, необходимо, чтобы $\ga_2$ из примера \ref{example2} была равна сумме $\ga_2$ и $\ga_3$ из примера \ref{example1}.
 \end{example}
 
 \begin{proposition}\label{prop multiplicativitycomp}
\begin{speqn}
 \varphi_{\wt{u}}\lr{M_{\la}M_{\mu}}=M^{\circ}_{\mu}(\ol{u})\varphi_{\wt{u}}\lr{M_{\la}},\ \text{если}\ \la\supseteq\la_{\wt{u}}\ \text{или}\ \la\notin\GK_{\wt{u}}.
 \end{speqn}
\end{proposition} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{"Проекция" на граф Кингмана.}
Каждая полуконечная гармоническая функция на графе $\GK$ задает аддитивное $\RR$ - линейное отображение \mbox{$K^{\qsym}\rightarrow \RR\cup\{+\Inf\}$}, где $K^{\qsym}$ -- положительный конус в $\qsym$, натянутый на мономиальные квазисимметрические функции $M_{\la}$. Каждое такое отображение можно ограничить на положительный конус $K^{\sym}\subset K^{\qsym}$, соответствующий мономиальным \textit{симметрическим} функциям $m_{\la}$. Тогда мы получим некоторую (бесконечную) гармоническую функцию на графе Кингмана.

Для описания этого ограничения нам потребуется следующий набор данных:
\begin{itemize}
    \item Набор невозрастающих положительных чисел -- набор длин $h$ - интервалов $\wt{u}$ взятых в порядке убывания длины. Обозначим этот невозрастающий набор через $\alpha_1,\ldots, \alpha_k$, а $\ga=1-\lr{\alpha_1+\ldots+\alpha_k}=\summ_{i}\ga_i$.
    
    \item "Нарост" в виде диаграммы Юнга -- все разделяющие композиции склеиваются в одну диаграмму Юнга. То есть они объединяются в одну композицию и потом ее строки упорядочиваются по убыванию длины сверху вниз. Обозначим эту диаграмму Юнга через $\nu$. 
\end{itemize}

Полуконечную гармоническую функцию на графе Кингмана, соответствующую набору $(\alpha, \nu)$ обозначим через $\varphi^{\king}_{\alpha,\nu}$, см. \cite{kerov_example}. 

\begin{proposition}\label{restriction from com to king}
\begin{speqn}
 \varphi_{\wt{u}}\lr{m_{\la}}=\varphi^{\mathbb{K}}_{\alpha,\nu}\lr{\la},\ \la\in\king,
\end{speqn}
если $\wt{u}$ не имел ни одного $v$ - интервала или никакая из разделяющих композиций не имела строк длины $1$. В противном случае
\begin{speqn}
 \varphi_{\wt{u}}\lr{m_{\la}}=\begin{cases}
 +\Inf, &\text{если}\ \varphi^{\king}_{\alpha,\nu}\lr{\la}\neq 0,\\
 0, &\text{иначе}.
 \end{cases}
\end{speqn}
\end{proposition}

Следует отметить, что во втором случае гармоническая функция не является полуконечной.

%мы получили заведомо разложимую гармоническую функцию на графе Кингмана, потому что $\varphi_{\wt{u}}{\big|}_{\mathbb{K}}\geq \varphi^{\mathbb{K}}_{\alpha,\nu}$, но они не пропорциональны.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Еще следует упомянуть дифференциальные операторы Вершика-Керова. В случае графа Гнедина-Кингмана их удается канонически построить только для одного конкретного случая -- когда $\wt{u}\in \wt{U}_0$ состоит из чередующегося набора интервалов и промежутков, окруженного с двух сторон композициями. Таким образом, разделяющие композиции находятся только в начале и конце единичного интервала, но не внутри. Обозначим эти композиции через $\nu_1,\nu_2$. Тогда
\begin{speqn}
    \varphi_{\wt{u}}(M_{\la})=\begin{cases}
    \varphi_{\ol{u}}\biglr{L^*_{\nu_1}R^*_{\nu_2}\lr{M_{\la}}}, &\text{если}\ \  \la\in\GK^{\la_{\wt{u}}}\cup \GK^{\wt{u}},\\
    +\Inf, &\text{иначе},
    \end{cases}
\end{speqn}
    где $\varphi_{\ol{u}}$ - конечный характер, соответствующий $\ol{u}$: $\la\mapsto M^{\circ}_{\la}(\ol{u})$, а $L^*_{\nu_1}$ и $R^*_{\nu_2}$ -- операторы $\qsym\rightarrow \qsym$, сопряженные к умножению справа и слева на $\h_{\nu_1}$ и $\h_{\nu_2}$ в алгебре некоммутативных симметрических функций $\nsym$:
    
    \begin{speqn}
    L_{\al}\lr{\h_{\beta}}=\h_{\al\sqcup \beta},\ \  R_{\al}\lr{\h_{\beta}}=\h_{\beta\sqcup \al},\\
    L_{\al}^*\lr{M_{\beta}}=\begin{cases}
    M_{\ga}, &\text{если}\ \beta=\al\sqcup\ga,\\
    0, &\text{иначе}
    \end{cases}
    ,\ \ R_{\al}^*\lr{M_{\beta}}=\begin{cases}
    M_{\ga}, &\text{если}\ \beta=\ga\sqcup\al,\\
    0, &\text{иначе}
    \end{cases}.
    \end{speqn}



\subsection{Некоторые разложимые гармонические функции}\label{the last section intro}
Теперь мы опишем некоторые разложимые гармонические функции, которые получаются из $\varphi_{\wt{u}}$ при помощи очевидной модификации.

Пусть $\wt{u}\in\wt{U}_0$ и $\nu\in\GK$ любая такая композиция, что $\nu\supseteq \la_{\wt{u}}$. Тогда мы определим гармоническую функцию $\varphi_{\wt{u}, \nu}$ следующим образом:
\begin{speqn}
\varphi_{\wt{u}, \nu}(\la)=\varphi_{\wt{u}}+\delta_{\nu}=\begin{cases}
 \lim\limits_{\varepsilon\to 0}\cfrac{1}{\eps^{|\la_{\wt{u}}|}}\cdot M^{\circ}_{\la}(\wt{u}^{\eps}), &\text{если}\ \la\supseteq \nu,\\
 +\Inf, &\text{иначе},
 \end{cases}
\end{speqn}
где 
\begin{speqn}
\delta_{\nu}(\la)=\begin{cases}
 0, &\text{если}\ \la\supseteq \nu,\\
 +\Inf, &\text{иначе}.
 \end{cases}
\end{speqn}

Например, $\delta_{(1)}=0$ и 
\begin{speqn}
    \delta_{(1,1)}(\la)=\begin{cases}
    +\Inf,\ &\text{если}\ \la=(n),\\
    
    0,\ &\text{иначе},
    \end{cases}\ \ \ \delta_{(2)}(\la)=\begin{cases}
    +\Inf\ ,\ &\text{если}\ \la=\underbrace{1,\ldots,1}_n,\\
    
    0,\ &\text{иначе}.
    \end{cases}
    \end{speqn}

\begin{proposition}
При каждом \mbox{$\nu\in \GK$} функция $\delta_{\nu}$ является полуконечной и гармонической.
\end{proposition}
\begin{remark}
Заметим, что $\delta_{\nu}$ не может быть неразложимой. Действительно, если $\nu_1<\nu_2$, то $\delta_{\nu_1}\geq \delta_{\nu_2}$ и $\delta_{(1,1)}\geq \psi_+$, $\delta_{(2)}\geq \psi_-$, где $\psi_+$ и $\psi_-$ определены равенствами \eqref{psi}.
\end{remark}

\begin{remark}\label{important remarkkk}
Для заведомо разложимых гармонических функций $\varphi_{\wt{u}, \nu}$ выполняется свойство мультипликативности:

\begin{speqn}
 \varphi_{\wt{u},\nu}\lr{M_{\la}M_{\mu}}=M^{\circ}_{\mu}(\ol{u})\varphi_{\wt{u},\nu}\lr{M_{\la}},\ \text{при}\ \la\supseteq\nu.
 \end{speqn}
\end{remark}


 


 \begin{definition}\label{def admissible words}
    Слово в алфавите $\Inf, \1, n$ при $n\in\Z_{\geq 1}$ называется \emph{шаблоном}, если выполняются следующие условия
    \begin{enumerate}
        \item два символа $\1$ не могут стоять рядом
        
        \item если символы $n$ и $\1$ стоят рядом, то $n\geq2$
        
        \item слово содержит по крайней мере один символ бесконечного типа, то есть $\Inf$ или $\1$.
    \end{enumerate}
    Будем говорить, что шаблон $t$ имеет \emph{первый тип}, если $t$ не содержит конечных символов и \emph{второй тип} иначе.
    \end{definition}
    
Шаблону соответствует коидеал в графе Гнедина-Кингмана $\GK_t=\bigcupp_{n}\{\la\in\GK\mid \la\subseteq t_n\}$, где $t_n$ - композиции, получающиеся из $t$ заменой $\Inf$ на $n$, а $\1$ на $\underbrace{1,\ldots,1}_{n}$.
    
По шаблону $t$ построим композицию по следующим правилам:
 \begin{enumerate}
     \item конечные символы слова $t$ остаются неизменными
     
     \item символ $\Inf$ заменяется на 
     \begin{itemize}
         \item $1$, если он не соседствовал с символом $1^{\Inf}$
         
         \item $2$, если соседствовал
     \end{itemize} 
     
     \item символы $\1$ удаляются.
 \end{enumerate}
 
 Выполнив эти действия в указанном порядке, мы получим некоторую композицию, которую обозначим через $\la_t$. Например, $t=(\1,\Inf,\Inf,5)$, $\la_t=(2,1,5)$.
 
 Композиция $\la_t$ может расти внутри $\GK_t$ очень ограниченным образом -- наросты могут появляться только на местах соответствующих символам $\Inf$ и $\1$ в шаблоне $t$. На месте символа $\Inf$ расти может строка, а на месте символа $\1$ -- столбец. Таким образом, мы можем отождествить вершины графа $\lr{\GK_t}^{\la_t}$ с вершинами пирамиды Паскаля подходящей размерности. Обозначим это отображение через $\lr{\GK_t}^{\la_t}\iso \Pas_m$, $\la\mapsto\la_{\pm}$. Набор чисел $\la_{\pm}$ мы можем разбить на два поднабора -- числа соответствующие символам $\Inf$ и символам $\1$. Первый набор чисел обозначим через $\la_+$, а второй через $\la_-$.
    

\begin{theorem}
    Пусть $\varphi$ -- полуконечный характер $\GK$. Тогда существует шаблон второго типа $t$ и положительные вещественные числа $u_1,\ldots u_m$, такие что $u_1+\ldots+ u_m=1$, $m$ -- число бесконечных символов $t$ и 
    \begin{speqn}
    \varphi(\la)=\begin{cases}
    \cfrac{1}{\lr{\la_-}!}\cdot u^{\la_{\pm}},\ \text{if}\ \la\in\GK_t,\ \la\supseteq{\la_t},\\
    +\infty,\ \la\in\GK_t,\ \la\nsupseteq\la_t,\\
    0,\ \la\notin\GK_t,
    \end{cases}
    \end{speqn}
    
   Мы пользуемся обозначениями $x!=x_1! x_2!\ldots $ и $x^{\nu}=x_1^{\nu_1}x_2^{\nu_2}\ldots$.  
\end{theorem}




\section{Дифференциальные операторы ВК}

Первым делом, напомним кое-что про алгебру некоммутативных симметрических функций $\nsym$. Рассмотрим операторы $R_{\alpha}$, $L_{\alpha}$ умножения справа и слева на $\h_{\alpha}=\h_{\al_1}\h_{\al_2}\ldots$, где $\h_{k}$ -- некоммутативная полная симметрическая функция, а $\al$ -- композиция. Обозначим через $R_{\alpha}^*$, $L_{\alpha}^*$ сопряженные операторы.
     
    \begin{speqn}
    L_{\al}\lr{\h_{\beta}}=\h_{\al\sqcup \beta},\ \  R_{\al}\lr{\h_{\beta}}=\h_{\beta\sqcup \al},\\
    L_{\al}^*\lr{M_{\beta}}=\begin{cases}
    M_{\ga},\ \ \text{if}\ \beta=\al\sqcup\ga,\\
    0,\ \ \text{otherwise}
    \end{cases}
    ,\ \ R_{\al}^*\lr{M_{\beta}}=\begin{cases}
    M_{\ga},\ \ \text{if}\ \beta=\ga\sqcup\al,\\
    0,\ \ \text{otherwise}
    \end{cases}.
    \end{speqn}
    
    \begin{example}
    Пусть $t=\nu_1\sqcup \tau \sqcup \nu_2$, где $\tau$ - шаблон первого типа, а $\nu_1,\nu_2\in\GK$. Тогда любой точный полуконечный характер $\GK_t$ имеет вид
    
    \begin{speqn}
    \varphi(M_{\la})=\begin{cases}
    \varphi_u\biglr{L^*_{\nu_1}R^*_{\nu_2}\lr{M_{\la}}},\ \ \text{if}\ \  \la\supseteq \la_t\\
    +\Inf, \ \ \text{otherwise},
    \end{cases}
    \end{speqn}
    где $\varphi_u$ - точный конечный характер $\GK_{\tau}$.
    \end{example}
    
Дальше мы опишем более общий результат, справедливый для любого шаблона второго типа. Для этого нам понадобится некоторый линейный оператор, который будет играть роль $L^*_{\nu_1}R^*_{\nu_2}$.

Каждый шаблон второго типа можно представить как склейку нескольких элементарных кусочков, каждый из которых имеет вид $\1$, $\underbrace{\Inf,
\ldots,\Inf}_{n}$ для некоторого $n$ или некоторой композиции. Каждому такому элементарному кусочку $\tau$ сопоставим счетный(или даже конечный) набор переменных $X_{\tau}$ следующим образом
    \begin{speqn}
    X_{\tau}=\begin{cases}
    \{x_{1},\ldots,x_{n}\},\ \text{if}\ \tau=(\overbrace{\Inf,\ldots,\Inf}^{n}),\ \text{for some}\ n\in\Z_{\geq 1}\\
    \{x_1,x_2,\ldots\},\ \text{where}\ \lr{x_i}^{2}=0,\ \text{if}\ \tau=\1,\\
    \{x_{1},x_{2},\ldots,x_{l}\},\ \text{where}\ l=l(\nu)\ \text{and}\ \lr{x_i}^{\nu_i+1}\!\!\!\!\!\!=0,\ \text{if}\ \tau=\nu\in\GK.
    \end{cases}
    \end{speqn}
    
    Через $X_t$ мы будем обозначать упорядоченный набор формальных переменных, соответствующих всем элементарным кусочкам шаблона $t$. Таким образом, мы каждой ''строчке'' шаблона $t$ сопоставили переменную. Переменная нильпотентна только если строчка конечна. Рассмотрим алгебру квазисимметрических функций $\qsym\lr{X_t}$ от переменных $X_t$. Базисом этой алгебры являются мономиальные квазисимметрические функции от переменных $X_t$. Отличие от $\qsym$ заключается в том, что в определении мономиальной квазисимметрической функции некоторые мономы обнуляются. Отметим, что $\qsym\lr{X_{\Inf}}\simeq \R[x]$. По определению также полагается $\qsym\lr{X_{\diameter}}=\R$.
    
    Обозначим через $t^{min}$\label{tmin} шаблон, который получается из $t$ по следующим правилам:
    \begin{enumerate}
        \item все конечные блоки $t$, не стоящие между двумя символами $\1$, удаляются
        
        \item конечные блоки, стоящие между двумя символами $\1$, заменяются на $(2)$.
    \end{enumerate}

Представим шаблон $t$ в виде $t=(t_1,t_2,\ldots, t_l)$, где $t_i$ - это или некоторая композиция, или шаблон первого типа.

    Введем обозначение
    \begin{speqn}
    t_i^{(m)}=\begin{cases}
    \diameter,\ &\text{if}\ t_i=\nu,\ \text{where}\ \nu\in\GK,\ \text{and}\ (t_{i-1},t_i,t_{i+1})\neq(\ldots,\1,\nu,\1,\ldots),\\
    (2),\ &\text{if}\ t_i=\nu,\ \text{where}\ \nu\in\GK,\ \text{and}\ (t_{i-1},t_i,t_{i+1})=(\ldots,\1,\nu,\1,\ldots), \\
    t_i,\ \ &\text{otherwise}.
    \end{cases}
    \end{speqn}
    
    Тогда можно написать $t^{min}=\lr{t_1^{(m)},t_2^{(m)},\ldots,t_l^{(m)}}$.
    
    Разделим переменные $X_t$ на несколько частей $X_{t_1}\sqcup\ldots\sqcup X_{t_l}$ в соответствии с $t=(t_1,t_2,\ldots, t_l)$.
    
    Определим линейные операторы $H^*_{t_i}\colon \qsym\lr{X_{t_i}}\rightarrow \qsym\lr{\!X_{t^{(m)}_i}\!}$ следующим образом
    \begin{speqn}
    H^*_{t_i}=\begin{cases}
    H^*_{\nu},\ &\text{if}\ t_i=\nu,\ \text{where}\ \nu\in\GK,\ \text{and}\ (t_{i-1},t_i,t_{i+1})\neq(\ldots,\1,\nu,\1,\ldots),\\
    M_{(2)}H^*_{\nu},\ &\text{if}\ t_i=\nu,\ \text{where}\ \nu\in\GK,\ \text{and}\ (t_{i-1},t_i,t_{i+1})=(\ldots,\1,\nu,\1,\ldots),\\
    1,\ &\text{otherwise},
    \end{cases}
    \end{speqn}
    где под $H^*_{\nu}$ можно понимать любой из операторов $R_{\nu}^*$, $L_{\nu}^*$, а под $M_{(2)}$ понимается оператор умножения на мономиальную квазисимметрическую функцию $M_{(2)}$.
    
    Рассмотрим оператор 
    \begin{speqn}
    H^*_{t_1}\otimes \ldots\otimes H^*_{t_l}\colon\qsym(X_{t_1})\otimes\ldots\otimes\qsym(X_{t_l})\longrightarrow\qsym(X_{t^{min}_1})\otimes\ldots\otimes\qsym(X_{t^{min}_l}).
    \end{speqn}
    
    Нетрудно увидеть, что его ограничение на $\qsym\lr{X_t}$ дает некоторый оператор $\qsym\lr{X_t}\rightarrow \qsym\lr{X_{t^{min}}}$. Введем обозначение
    \begin{speqn}\label{diff operator}
    H_t^*\colon \qsym\xrightarrowdbl{\ \ \pi_t\ } \qsym\lr{X_t}\rightarrow \qsym\lr{X_{t^{min}}},\\
    H_t^*=H^*_{t_1}\otimes H^*_{t_2}\otimes \ldots\otimes H^*_{t_l}\Big|_{\qsym\lr{X_t}}\circ \pi_t,
    \end{speqn}
    где $\pi_t$ - отображение факторизации.
    
    \begin{proposition}
   Все полуконечные характеры $\GK$ имеют вид
    \begin{speqn}
    \varphi(M_{\la})=\begin{cases}
    \varphi_u\lr{H_t^*M_{\la}},\ \ \text{if}\ \  \la\supseteq\la_t,\\
    +\Inf, \ \ \text{otherwise},
    \end{cases}
    \end{speqn}
    где $t$ -- некоторый шаблон второго типа, $\varphi_u$ -- точный полуконечный характер $\GK_{t^{min}}$.
    \end{proposition}



\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> 0_Main_results/temp.tex <==


 \section{Предел $\eps\to0$ не чувствует идеал конечности}
 Пусть $\wt{u}$ имеет следующий вид
 \begin{figure}[H]
     \centering
     

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_81t0w68xt}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_81t0w68xt}
{\pgfqpoint{0pt}{0pt}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{\mcSize+\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da4416939916397159] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (446.5,178) -- (482,178) ;
\draw [shift={(482,178)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(446.5,178)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
%Straight Lines [id:da4492772860083677] 
\draw [pattern=_81t0w68xt,pattern size=6pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] [dash pattern={on 0.84pt off 2.51pt}]  (571,140) -- (571.5,175.35) ;
%Straight Lines [id:da6093375162801964] 
\draw    (482,178) -- (571.5,178) ;

% Text Node
\draw (443.93,190) node [anchor=north west][inner sep=0.75pt]   [align=left] {0};
% Text Node
\draw (566,190) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (458.75,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (508.92,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1-\alpha $};
% Text Node
\draw (560,119.98) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle ( 2)$};


\end{tikzpicture}
 \end{figure}
 
 В этом случае $u^{\eps}$ имеет вид 
 \begin{figure}[H]
     \centering
    

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da4416939916397159] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (446.5,178) -- (482,178) ;
\draw [shift={(482,178)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(446.5,178)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
%Straight Lines [id:da6093375162801964] 
\draw    (482,178) -- (571.5,178) ;
%Straight Lines [id:da985123369815074] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (571.5,178) -- (589,178) ;
\draw [shift={(589,178)}, rotate = 180] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(571.5,178)}, rotate = 0] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;

% Text Node
\draw (458.75,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \alpha $};
% Text Node
\draw (508.92,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1-\alpha $};
% Text Node
\draw (576.5,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \varepsilon $};


\end{tikzpicture}
 \end{figure}
 
 Кроме того, $\la_{\wt{u}}=(2,2)$ и $\com_{\wt{u}}$, $\com_{u^{\eps}}$ имеют следующий вид. Штрихованными клетками обозначена композиция $\la_{\wt{u}}$.
 \begin{figure}[H]
     \centering
     

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_06n17o4wh}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_06n17o4wh}
{\pgfqpoint{0pt}{-\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_fkmuqmbwq}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_fkmuqmbwq}
{\pgfqpoint{0pt}{-\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_f66wisa4f}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_f66wisa4f}
{\pgfqpoint{0pt}{-\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother

% Pattern Info
 
\tikzset{
pattern size/.store in=\mcSize, 
pattern size = 5pt,
pattern thickness/.store in=\mcThickness, 
pattern thickness = 0.3pt,
pattern radius/.store in=\mcRadius, 
pattern radius = 1pt}
\makeatletter
\pgfutil@ifundefined{pgf@pattern@name@_kmnw1ya65}{
\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_kmnw1ya65}
{\pgfqpoint{0pt}{-\mcThickness}}
{\pgfpoint{\mcSize}{\mcSize}}
{\pgfpoint{\mcSize}{\mcSize}}
{
\pgfsetcolor{\tikz@pattern@color}
\pgfsetlinewidth{\mcThickness}
\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
\pgfusepath{stroke}
}}
\makeatother
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,191); %set diagram left start at 0, and has height of 191

%Shape: Grid [id:dp4492154315385656] 
\draw  [draw opacity=0][pattern=_06n17o4wh,pattern size=3pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (153.5,74.75) -- (173.5,74.75) -- (173.5,84.75) -- (153.5,84.75) -- cycle ; \draw   (163.5,74.75) -- (163.5,84.75) ; \draw    ; \draw   (153.5,74.75) -- (173.5,74.75) -- (173.5,84.75) -- (153.5,84.75) -- cycle ;
%Shape: Grid [id:dp22665269077212125] 
\draw  [draw opacity=0][pattern=_fkmuqmbwq,pattern size=3pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (153.5,164.75) -- (173.5,164.75) -- (173.5,174.75) -- (153.5,174.75) -- cycle ; \draw   (163.5,164.75) -- (163.5,174.75) ; \draw    ; \draw   (153.5,164.75) -- (173.5,164.75) -- (173.5,174.75) -- (153.5,174.75) -- cycle ;
%Shape: Grid [id:dp017762922552012284] 
\draw  [draw opacity=0] (173.5,74.75) -- (293.5,74.75) -- (293.5,84.75) -- (173.5,84.75) -- cycle ; \draw   (183.5,74.75) -- (183.5,84.75)(193.5,74.75) -- (193.5,84.75)(203.5,74.75) -- (203.5,84.75)(213.5,74.75) -- (213.5,84.75)(223.5,74.75) -- (223.5,84.75)(233.5,74.75) -- (233.5,84.75)(243.5,74.75) -- (243.5,84.75)(253.5,74.75) -- (253.5,84.75)(263.5,74.75) -- (263.5,84.75)(273.5,74.75) -- (273.5,84.75)(283.5,74.75) -- (283.5,84.75) ; \draw    ; \draw   (173.5,74.75) -- (293.5,74.75) -- (293.5,84.75) -- (173.5,84.75) -- cycle ;
%Shape: Grid [id:dp6433451751969157] 
\draw  [draw opacity=0] (153.5,84.75) -- (163.5,84.75) -- (163.5,164.75) -- (153.5,164.75) -- cycle ; \draw    ; \draw   (153.5,94.75) -- (163.5,94.75)(153.5,104.75) -- (163.5,104.75)(153.5,114.75) -- (163.5,114.75)(153.5,124.75) -- (163.5,124.75)(153.5,134.75) -- (163.5,134.75)(153.5,144.75) -- (163.5,144.75)(153.5,154.75) -- (163.5,154.75) ; \draw   (153.5,84.75) -- (163.5,84.75) -- (163.5,164.75) -- (153.5,164.75) -- cycle ;
%Shape: Grid [id:dp3599162572119816] 
\draw  [draw opacity=0][pattern=_f66wisa4f,pattern size=3pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (393.5,74.75) -- (413.5,74.75) -- (413.5,84.75) -- (393.5,84.75) -- cycle ; \draw   (403.5,74.75) -- (403.5,84.75) ; \draw    ; \draw   (393.5,74.75) -- (413.5,74.75) -- (413.5,84.75) -- (393.5,84.75) -- cycle ;
%Shape: Grid [id:dp038006079632298184] 
\draw  [draw opacity=0] (413.5,164.75) -- (533.5,164.75) -- (533.5,174.75) -- (413.5,174.75) -- cycle ; \draw   (423.5,164.75) -- (423.5,174.75)(433.5,164.75) -- (433.5,174.75)(443.5,164.75) -- (443.5,174.75)(453.5,164.75) -- (453.5,174.75)(463.5,164.75) -- (463.5,174.75)(473.5,164.75) -- (473.5,174.75)(483.5,164.75) -- (483.5,174.75)(493.5,164.75) -- (493.5,174.75)(503.5,164.75) -- (503.5,174.75)(513.5,164.75) -- (513.5,174.75)(523.5,164.75) -- (523.5,174.75) ; \draw    ; \draw   (413.5,164.75) -- (533.5,164.75) -- (533.5,174.75) -- (413.5,174.75) -- cycle ;
%Shape: Grid [id:dp7604789331245645] 
\draw  [draw opacity=0][pattern=_kmnw1ya65,pattern size=3pt,pattern thickness=0.75pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}] (393.5,164.75) -- (413.5,164.75) -- (413.5,174.75) -- (393.5,174.75) -- cycle ; \draw   (403.5,164.75) -- (403.5,174.75) ; \draw    ; \draw   (393.5,164.75) -- (413.5,164.75) -- (413.5,174.75) -- (393.5,174.75) -- cycle ;
%Shape: Grid [id:dp812131682933679] 
\draw  [draw opacity=0] (413.5,74.75) -- (533.5,74.75) -- (533.5,84.75) -- (413.5,84.75) -- cycle ; \draw   (423.5,74.75) -- (423.5,84.75)(433.5,74.75) -- (433.5,84.75)(443.5,74.75) -- (443.5,84.75)(453.5,74.75) -- (453.5,84.75)(463.5,74.75) -- (463.5,84.75)(473.5,74.75) -- (473.5,84.75)(483.5,74.75) -- (483.5,84.75)(493.5,74.75) -- (493.5,84.75)(503.5,74.75) -- (503.5,84.75)(513.5,74.75) -- (513.5,84.75)(523.5,74.75) -- (523.5,84.75) ; \draw    ; \draw   (413.5,74.75) -- (533.5,74.75) -- (533.5,84.75) -- (413.5,84.75) -- cycle ;
%Shape: Grid [id:dp5932259755881539] 
\draw  [draw opacity=0] (393.5,84.75) -- (403.5,84.75) -- (403.5,164.75) -- (393.5,164.75) -- cycle ; \draw    ; \draw   (393.5,94.75) -- (403.5,94.75)(393.5,104.75) -- (403.5,104.75)(393.5,114.75) -- (403.5,114.75)(393.5,124.75) -- (403.5,124.75)(393.5,134.75) -- (403.5,134.75)(393.5,144.75) -- (403.5,144.75)(393.5,154.75) -- (403.5,154.75) ; \draw   (393.5,84.75) -- (403.5,84.75) -- (403.5,164.75) -- (393.5,164.75) -- cycle ;

% Text Node
\draw (218,39) node [anchor=north west][inner sep=0.75pt]    {$\com_{\wt{u}} $};
% Text Node
\draw (457,39) node [anchor=north west][inner sep=0.75pt]    {$\com_{u^{\eps}}$};


\end{tikzpicture}
 \end{figure}
 
 
 Пусть $\la=(1,2)$. Тогда $\la\in\com_{\wt{u}}$, но $\la$ не содержит $\la_{\wt{u}}$ и должно быть $\varphi_{\wt{u}}(\la)=+\Inf$.
 
 С другой стороны,
 \begin{speqn}
 \M_{\la}(u^{\eps})=\al\eps^2+(1-\al)\eps^2=\eps^2.
 \end{speqn}
 
 Тогда 
 
 \begin{speqn}
 \cfrac{1}{\eps^2}\M_{\la}(u^{\eps})=1.
 \end{speqn}
 
 Причин делить на $\eps$ в какой-то другой степени, отличной от суммы весов разделяющих композиций(в нашем случае это $2$), вроде бы, нет.




\section{Предел $\eps\to0$ не чувствует множество нулей}
Пусть $\wt{u}$ имеет следующий вид
 \begin{figure}[H]
     \centering
     \import{/0_Main_results}{Picture_5}
 \end{figure}
 
 В этом случае $u^{\eps}$ имеет вид 
 \begin{figure}[H]
     \centering
     

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5344889164769645] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ]   (262.5,149) -- (365.75,149) ;
\draw [shift={(365.75,149)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(262.5,149)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
%Straight Lines [id:da32413284719249635] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (227.5,149) -- (245,149) ;
\draw [shift={(245,149)}, rotate = 180] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(227.5,149)}, rotate = 0] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;

%Straight Lines [id:da16856014619121606] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (245,149) -- (262.5,149) ;
\draw [shift={(262.5,149)}, rotate = 180] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;
\draw [shift={(245,149)}, rotate = 0] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]      (5.59,-5.59) .. controls (2.5,-5.59) and (0,-3.09) .. (0,0) .. controls (0,3.09) and (2.5,5.59) .. (5.59,5.59) ;



% Text Node
\draw (307.6,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle 1$};
% Text Node
\draw (249,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \varepsilon_2 $};
% Text Node
\draw (228,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \varepsilon_1\ $};


\end{tikzpicture}
 \end{figure}
 
 Кроме того, $\la_{\wt{u}}=(3,1,1)$ и $\com_{\wt{u}}$, $\com_{u^{\eps}}$ имеют следующий вид. Штрихованными клетками обозначена композиция $\la_{\wt{u}}$.
 \begin{figure}[H]
     \centering
     \import{0_Main_results}{Picture_6}
 \end{figure}
 
 
 Пусть $\la=(4,2)$. Тогда $\la\notin\com_{\wt{u}}$ и должно быть $\varphi_{\wt{u}}(\la)=0$.
 
 С другой стороны,
 \begin{speqn}
 \M_{\la}(u^{\eps})=\eps_1^4\eps_2^2+\eps_2^4+\eps_2^4.
 \end{speqn}
 
 Тогда 
 
 \begin{speqn}
 \cfrac{1}{\eps_1^3\eps_2}\M_{\la}(u^{\eps})=\eps_1\eps_2+\cfrac{\eps_1}{\eps_2}+\cfrac{\eps_2^3}{\eps_1^3}.
 \end{speqn}
 
 Последнее выражение никак не может стремиться к нулю при $\eps_1,\eps_2\to 0$ из-за последних двух слагаемых.  
 
 
 
